Universal Entanglement Distillation

We present a universal entanglement distillation protocol that asymptotically achieves the distillable entanglement of any unknown bipartite state in a fixed finite dimension. That is, its ebit yield attains every rate below the optimum that would be available if the state were known, with vanishing trace-distance error. Our approach combines tomography by local operations and classical communication with an adaptive distillation routine, using a local robustness lemma to control finite-sample estimation errors. We also characterize worst-case distillation from a family of states: the optimal uniform rate is the minimum distillable entanglement on the family's closure. These results show that ignorance of the state need not incur an asymptotic rate penalty.

==> newdef.tex <==
% Mathematical content and the original macro names are preserved.
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage{comment}
\usepackage{hyperref}

\newtheorem{thm}{Theorem}
\newtheorem{lemma}[thm]{Lemma}
\newcommand{\pazocal}{\mathcal}
\newcommand{\HH}{\pazocal{H}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\locc}{\mathrm{LOCC}}
\newcommand{\e}{\varepsilon}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\id}{\mathds{1}}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\ket}[1]{\lvert #1\rangle}
\newcommand{\bra}[1]{\langle #1\rvert}
\newcommand{\ketbra}[1]{\ket{#1}\!\bra{#1}}
\newcommand{\ketbraa}[2]{\ket{#1}\!\bra{#2}}
\newcommand{\ceil}[1]{\lceil #1\rceil}
\newcommand{\floor}[1]{\lfloor #1\rfloor}
\newcommand{\bb}{\begin{equation}\begin{aligned}}
\newcommand{\ee}{\end{aligned}\end{equation}}
\newcommand{\bbb}{\begin{equation*}\begin{aligned}}
\newcommand{\eee}{\end{aligned}\end{equation*}}

